Near-IR studies of recurrent nova V745 Scorpii during its 2014 outburst

The recurrent nova (RN) V745 Scorpii underwent its third known outburst on 2014 February 6. Infrared monitoring of the eruption on an almost daily basis, starting from 1.3d after discovery, shows the emergence of a powerful blast wave generated by the high velocity nova ejecta exceeding 4000 kms$^{-1}$ plowing into its surrounding environment. The temperature of the shocked gas is raised to a high value exceeding 10$^{8}$K immediately after outburst commencement. The energetics of the outburst clearly surpass those of similar symbiotic systems like RS Oph and V407 Cyg which have giant secondaries. The shock does not show a free-expansion stage but rather shows a decelerative Sedov-Taylor phase from the beginning. Such strong shockfronts are known to be sites for $\gamma$ ray generation. V745 Sco is the latest nova, apart from five other known novae, to show $\gamma$ ray emission. It may be an important testbed to resolve the crucial question whether all novae are generically $\gamma$ ray emitters by virtue of having a circumbinary reservoir of material that is shocked by the ejecta rather than $\gamma$ ray generation being restricted to only symbiotic systems with a shocked red giant (RG) wind. The lack of a free-expansion stage favors V745 Sco to have a density enhancement around the white dwarf (WD), above that contributed by a RG wind. Our analysis also suggests that the WD in V745 Sco is very massive and a potential progenitor for a future SN Ia explosion.

==> table.tex <==
4808.6392	&(	0	2	0	)[	19	0	19	]&(	0	3	1	)[	18	0	18	]&	4906.0562	&(	0	2	0	)[	15	1	14	]&(	0	3	1	)[	14	1	13	]	\\
4827.4287	&(	0	1	0	)[	20	1	20	]&(	0	2	1	)[	19	1	19	]&	4910.7778	&(	0	1	0	)[	17	2	15	]&(	0	2	1	)[	16	2	14	]	\\
4832.6523	&(	0	2	0	)[	18	1	18	]&(	0	3	1	)[	17	1	17	]&	4912.0356	&(	0	0	0	)[	19	1	18	]&(	0	1	1	)[	18	1	17	]	\\
4845.3232	&(	0	0	0	)[	21	0	21	]&(	0	1	1	)[	20	0	20	]&	4912.209	&(	0	1	0	)[	17	1	16	]&(	0	2	1	)[	16	1	15	]	\\
4852.9321	&(	0	1	0	)[	19	0	19	]&(	0	2	1	)[	18	0	18	]&	4923.124	&(	0	3	0	)[	12	2	11	]&(	0	4	1	)[	11	2	10	]	\\
4854.6118	&(	0	3	0	)[	15	0	15	]&(	0	4	1	)[	14	0	14	]&	4923.3872	&(	0	3	0	)[	12	1	12	]&(	0	4	1	)[	11	1	11	]	\\
4856.6558	&(	0	2	0	)[	17	0	17	]&(	0	3	1	)[	16	0	16	]&	4923.8242	&(	0	1	0	)[	15	4	11	]&(	0	2	1	)[	14	4	10	]	\\
4867.0205	&(	0	2	0	)[	17	1	16	]&(	0	3	1	)[	16	1	15	]&	4924.6816	&(	0	0	0	)[	18	1	18	]&(	0	1	1	)[	17	1	17	]	\\
4867.6724	&(	0	1	0	)[	19	1	18	]&(	0	2	1	)[	18	1	17	]&	4925.189	&(	0	2	0	)[	14	3	12	]&(	0	3	1	)[	13	3	11	]	\\
4872.1045	&(	0	0	0	)[	20	1	20	]&(	0	1	1	)[	19	1	19	]&	4927.5957	&(	0	1	0	)[	16	1	16	]&(	0	2	1	)[	15	1	15	]	\\
4878.1919	&(	0	1	0	)[	18	1	18	]&(	0	2	1	)[	17	1	17	]&	4927.9546	&(	0	1	0	)[	16	4	13	]&(	0	2	1	)[	15	4	12	]	\\
4879.4023	&(	0	2	0	)[	16	1	16	]&(	0	3	1	)[	15	1	15	]&	4928.3613	&(	0	2	0	)[	14	1	14	]&(	0	3	1	)[	13	1	13	]	\\
4880.5835	&(	0	3	0	)[	14	1	14	]&(	0	4	1	)[	13	1	13	]&	4930.9028	&(	0	2	0	)[	14	2	13	]&(	0	3	1	)[	13	2	12	]	\\
4889.8496	&(	0	1	0	)[	18	2	17	]&(	0	2	1	)[	17	2	16	]&	4933.3892	&(	0	1	0	)[	16	3	14	]&(	0	2	1	)[	15	3	13	]	\\
4890.4746	&(	0	2	0	)[	16	2	15	]&(	0	3	1	)[	15	2	14	]&	4935.5469	&(	0	2	0	)[	13	2	11	]&(	0	3	1	)[	12	2	10	]	\\
4898.5664	&(	0	0	0	)[	19	0	19	]&(	0	1	1	)[	18	0	18	]&	4935.5898	&(	0	0	0	)[	18	2	17	]&(	0	1	1	)[	17	2	16	]	\\
4900.6553	&(	0	2	0	)[	15	2	13	]&(	0	3	1	)[	14	2	12	]&	4936.0659	&(	0	1	0	)[	16	2	15	]&(	0	2	1	)[	15	2	14	]	\\
4903.1157	&(	0	1	0	)[	17	0	17	]&(	0	2	1	)[	16	0	16	]&	4937.2256	&(	0	3	0	)[	11	1	10	]&(	0	4	1	)[	10	1	9	]	\\
4903.1504	&(	0	2	0	)[	15	0	15	]&(	0	3	1	)[	14	0	14	]&	4939.376	&(	0	1	0	)[	15	3	12	]&(	0	2	1	)[	14	3	11	]	\\
4905.0444	&(	0	3	0	)[	13	0	13	]&(	0	4	1	)[	12	0	12	]&	4944.5679	&(	0	3	0	)[	11	0	11	]&(	0	4	1	)[	10	0	10	]	\\
